Oolong: Investigating What Makes Transfer Learning Hard with Controlled Studies

When we transfer a pretrained language model to a new language, there are many axes of variation that change at once. To disentangle the impact of different factors like syntactic similarity and vocabulary similarity, we propose a set of controlled transfer studies: we systematically transform the language of the GLUE benchmark, altering one axis of crosslingual variation at a time, and then measure the resulting drops in a pretrained model's downstream performance. We find that models can largely recover from syntactic-style shifts, but cannot recover from vocabulary misalignment and embedding matrix re-initialization, even with continued pretraining on 15 million tokens. %On the other hand, transferring to a dataset with an unaligned vocabulary is extremely hard to recover from in the low-data regime. Moreover, good-quality tokenizers in the transfer language do not make vocabulary alignment easier. Our experiments provide insights into the factors of cross-lingual transfer that researchers should most focus on when designing language transfer scenarios.

==> figures/deberta-xlmr-single-seed-no-midtune.tex <==
\begin{figure*}[tb]
  \centering
  \includegraphics[width=1.0\textwidth]{figures/deberta-xlmr-single-seed-no-midtune.png}
  \caption{GLUE scores for t-Englishes with scrambled word identities, syntactic shifts, tokenizer substitutions and original English without continued pretraining.}
  \label{fig:deberta-xlmr}
\end{figure*}

